Terahertz scale microbunching instability driven by nonevaporable getter coating resistive-wall impedance

Non-evaporable getter (NEG) coating is widely required in the next generation of light sources and circular $e^+e^-$ colliders for small vacuum pipes to improve the vacuum level, which, however, also enhances the high-frequency resistive-wall impedance and often generates a resonator-like peak in the terahertz frequency region. In this paper, we will use the parameters of the planned Hefei Advanced Light Facility (HALF) storage ring to study the impact of NEG coating resistive-wall impedance on the longitudinal microwave instability via particle tracking simulation. Using different NEG coating parameters (resistivity and thickness) as examples, we find that the impedance with a narrow and strong peak in the high frequency region can cause micro-bunching instability, which has a low instability threshold current and contributes to a large energy spread widening above the threshold. In order to obtain a convergent simulation of the beam dynamics, one must properly resolve such a peak. The coating with a lower resistivity has a much less sharp peak in its impedance spectrum, which is helpful to suppress the micro-bunching instability and in return contributes to a weaker microwave instability.

==> ref <==
@inbook{Malyshev2019,
author = {Malyshev, Oleg B.},
publisher = {John Wiley & Sons, Ltd},
isbn = {9783527809134},
title = {Non-evaporable Getter ({NEG})-Coated Vacuum Chamber},
booktitle = {Vacuum in Particle Accelerators},
chapter = {5},
pages = {175-213},
doi = {https://doi.org/10.1002/9783527809134.ch5},
url = {https://onlinelibrary.wiley.com/doi/abs/10.1002/9783527809134.ch5},
year = {2019},
keywords = {ion-stimulated desorption, non-evaporable getter coatings, particle accelerators, photon stimulated desorption, physical vapour deposition, reduced particle stimulated desorption: electron stimulated desorption, reduced thermal outgassing},
}

@article{Nagaoka2014,
author = "Nagaoka, Ryutaro and Bane, Karl L. F.",
title = "{Collective effects in a diffraction-limited storage~ring}",
journal = "Journal of Synchrotron Radiation",
year = "2014",
volume = "21",
number = "5",
pages = "937--960",
month = "Sep",
doi = {10.1107/S1600577514015215},
url = {https://doi.org/10.1107/S1600577514015215},
abstract = {This paper gives an overview of collective effects that are likely to appear and possibly limit the performance in a diffraction-limited storage ring (DLSR) that stores a high-intensity ultra-low-emittance beam. Beam instabilities and other intensity-dependent effects that may significantly impact the machine performance are covered. The latter include beam-induced machine heating, Touschek scattering, intra-beam scattering, as well as incoherent tune shifts. The general trend that the efforts to achieve ultra-low emittance result in increasing the machine coupling impedance and the beam sensitivity to instability is reviewed. The nature of coupling impedance in a DLSR is described, followed by a series of potentially dangerous beam instabilities driven by the former, such as resistive-wall, TMCI (transverse mode coupling instability), head{--}tail and microwave instabilities. In addition, beam-ion and CSR (coherent synchrotron radiation) instabilities are also treated. Means to fight against collective effects such as lengthening of the bunch with passive harmonic cavities and bunch-by-bunch transverse feedback are introduced. Numerical codes developed and used to evaluate the machine coupling impedance, as well as to simulate beam instability using the former as inputs are described.},
keywords = {diffraction-limited storage ring, beam instability, collective effects, wake function, impedance, low emittance, light source},
}

@article{Blednykh2021,
  title = {Impedance modeling and its application to the analysis of the collective effects},
  author = {Blednykh, A. and Bassi, G. and Smaluk, V. and Lindberg, R.},
  journal = {Phys. Rev. Accel. Beams},
  volume = {24},
  issue = {10},
  pages = {104801},
  numpages = {22},
  year = {2021},
  month = {Oct},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevAccelBeams.24.104801},
  url = {https://link.aps.org/doi/10.1103/PhysRevAccelBeams.24.104801}
}


@article{Migliorati2018,
  title = {Impact of the resistive wall impedance on beam dynamics in the Future Circular ${e}^{+}{e}^{\ensuremath{-}}$ Collider},
  author = {Migliorati, M. and Belli, E. and Zobov, M.},
  journal = {Phys. Rev. Accel. Beams},
  volume = {21},
  issue = {4},
  pages = {041001},
  numpages = {12},
  year = {2018},
  month = {Apr},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevAccelBeams.21.041001},
  url = {https://link.aps.org/doi/10.1103/PhysRevAccelBeams.21.041001}
}

@inproceedings{wang2022,
  author       = {N. Wang and C.T. Lin and Y.D. Liu and S.K. Tian and H.S. Xu and Y. Zhang},
  title        = {Collective Effects Studies for {CEPC}},
  booktitle    = "Proc. 65th ICFA Adv. Beam Dyn. Workshop High Luminosity Circular e+e- Colliders (eeFACT'22)",
  pages        = {141--145},
  eid          = {WEYAT0101},
  keywords     = {impedance, vacuum, coupling, synchrotron, simulation},
  venue        = {Frascati, Italy},
  series       = {ICFA Advanced Beam Dynamics Workshop on High Luminosity Circular e+e- Colliders},
  number       = {65},
  publisher    = {JACoW Publishing, Geneva, Switzerland},
  month        = {02},
  year         = {2022},
  issn         = {2673-7027},
  isbn         = {978-3-95450-236-3},
  doi          = {10.18429/JACoW-eeFACT2022-WEYAT0101},
  url          = {https://jacow.org/eefact2022/papers/weyat0101.pdf},
}

@InProceedings{WangNa2017,
  author       = {N. Wang and Z. Duan and X.Y. Li and H. Shi and S.K. Tian and G. Xu},
  title        = {{D}evelopment of the {I}mpedance {M}odel in {HEPS}},
  booktitle    = {Proc. of International Particle Accelerator Conference (IPAC'17),
                  Copenhagen, Denmark, 14-19 May, 2017},
  pages        = {3110--3113},
  paper        = {WEPIK078},
  keywords     = {impedance, vacuum, kicker, injection, feedback},
  venue        = {Copenhagen, Denmark},
  series       = {International Particle Accelerator Conference},
  number       = {8},
  publisher    = {JACoW},
  address      = {Geneva, Switzerland},
  month        = {May},
  year         = {2017},
  isbn         = {978-3-95450-182-3},
  doi          = {https://doi.org/10.18429/JACoW-IPAC2017-WEPIK078},
  url          = {http://jacow.org/ipac2017/papers/wepik078.pdf},
  note         = {https://doi.org/10.18429/JACoW-IPAC2017-WEPIK078},
}

@InProceedings{Dehler2019,
  author       = {M.M. Dehler and others},
  title        = {{C}haracterization of {NEG} {C}oatings for {SLS} 2.0},
  booktitle    = {Proc. 10th International Particle Accelerator Conference (IPAC'19),
                  Melbourne, Australia, 19-24 May 2019},
  pages        = {1662--1665},
  paper        = {TUPGW108},
  keywords     = {GUI, impedance, resonance, coupling, vacuum},
  venue        = {Melbourne, Australia},
  series       = {International Particle Accelerator Conference},
  number       = {10},
  publisher    = {JACoW Publishing},
  address      = {Geneva, Switzerland},
  month        = {Jun.},
  year         = {2019},
  isbn         = {978-3-95450-208-0},
  doi          = {doi:10.18429/JACoW-IPAC2019-TUPGW108},
  url          = {http://jacow.org/ipac2019/papers/tupgw108.pdf},
  note         = {https://doi.org/10.18429/JACoW-IPAC2019-TUPGW108},
}

@InProceedings{Plouviez2018,
  author       = {E. Plouviez},
  title        = {Comments on resistive measurement of {NEG} coated surface},
  booktitle    = {7th Low Emittance Rings Workshop },
  address      = {CERN},
  year         = {2018},
  url          ={https://indico.cern.ch/event/671745/contributions/2844086/},
}

@article{Gamelin2023,
  title = {Influence of the coating resistivity on beam dynamics},
  author = {Gamelin, A. and Foosang, W.},
  journal = {Phys. Rev. Accel. Beams},
  volume = {26},
  issue = {5},
  pages = {054401},
  numpages = {11},
  year = {2023},
  month = {May},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevAccelBeams.26.054401},
  url = {https://link.aps.org/doi/10.1103/PhysRevAccelBeams.26.054401}
}


@article{Shobuda2017,
    author = {Shobuda, Yoshihiro and Chin, Yong Ho},
    title = "{Resistive-wall impedances of a thin non-evaporable getter coating on a conductive chamber}",
    journal = {Progress of Theoretical and Experimental Physics},
    volume = {2017},
    number = {12},
    pages = {123G01},
    year = {2017},
    month = {12},
    abstract = "{The resistive-wall impedances of a thin non-evaporable getter (NEG) with constant conductivity coating on a copper chamber are studied in both longitudinal and transverse directions. The copper chamber has a finite thickness and is surrounded by air. As the frequency increases, wake fields see mostly the air first and then the copper chamber next, and then finally the NEG coating. Both longitudinal and transverse impedances slowly undergo transitions from the resistive-wall impedances of the copper-only chamber to those of the NEG-only chamber over a 0.1–100 GHz frequency range. They start to deviate from the conventional impedance lines for the NEG-only chamber at \\$\\sim\\$100 GHz. They increase first to \\$\\sim\\$1 THz and then decrease rapidly as a function of the frequency. Numerical examples of the resistive-wall impedances are presented up to \\$\\sim\\$100 THz using similar parameters to those of the SLS-II (Swiss Light Source) upgrade. We briefly discuss the characteristic of a loss factor for the chamber with NEG coating.}",
    issn = {2050-3911},
    doi = {10.1093/ptep/ptx167},
    url = {https://doi.org/10.1093/ptep/ptx167},
    eprint = {https://academic.oup.com/ptep/article-pdf/2017/12/123G01/22759002/ptx167.pdf},
}

@article{Motlagh2023,
  doi = {10.1088/1748-0221/18/01/P01028},
  url = {https://dx.doi.org/10.1088/1748-0221/18/01/P01028},
  year = {2023},
  month = {jan},
  publisher = {IOP Publishing},
  volume = {18},
  number = {01},
  pages = {P01028 (2023)},
  author = {S. Talebi Motlagh and J. Rahighi and F. Zamani and F. Saeidi},
  title = {The resistive wall impedance and the effects of the non-evaporable getter thickness in an ultra-low emittance ring},
  journal = {Journal of Instrumentation},
   abstract = {In modern particle accelerators with ultra-low emittance, the vacuum chambers are designed based on Non-Evaporable Getter (NEG)-coated vacuum chambers. The thickness of the NEG coating plays a critical role in the dynamic beam effects. So, in this paper, the longitudinal and transverse impedance of a copper chamber coated with a NEG are investigated, and the effects of the NEG thickness over a wide range of frequencies have been studied. A good selection of NEG layer thickness could minimize the coating effects on the longitudinal and transverse beam impedance. The numerical results in this work show that the beam dynamic effects could be minimal with selecting a NEG coating thickness of about 1 μm.}
}

@article{Bassi2016,
  title = {Self-consistent simulations and analysis of the coupled-bunch instability for arbitrary multibunch configurations},
  author = {Bassi, Gabriele and Blednykh, Alexei and Smaluk, Victor},
  journal = {Phys. Rev. Accel. Beams},
  volume = {19},
  issue = {2},
  pages = {024401},
  numpages = {20},
  year = {2016},
  month = {Feb},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevAccelBeams.19.024401},
  url = {https://link.aps.org/doi/10.1103/PhysRevAccelBeams.19.024401}
}



@misc{PyHEADTAIL,
  howpublished = {\url{https://github.com/PyCOMPLETE/PyHEADTAIL.}}
}

@article{SKRIPKA2016,
title = {Simultaneous computation of intrabunch and interbunch collective beam motions in storage rings},
journal = {Nuclear Instruments and Methods in Physics Research Section A: Accelerators, Spectrometers, Detectors and Associated Equipment},
volume = {806},
pages = {221-230},
year = {2016},
issn = {0168-9002},
doi = {https://doi.org/10.1016/j.nima.2015.10.029},
url = {https://www.sciencedirect.com/science/article/pii/S016890021501236X},
author = {Galina Skripka and Ryutaro Nagaoka and Marit Klein and Francis Cullinan and Pedro F. Tavares},
keywords = {Particle tracking code, Collective effects, Storage rings, Wakefields},
abstract = {We present the multibunch tracking code mbtrack developed to simulate, in 6-dimensional phase space, single- and multibunch collective instabilities driven by short- and long-range wakefields in storage rings. Multiple bunches, each composed of a large number of macroparticles, are tracked, allowing simulation of both intra- and interbunch motions. Besides analytical impedance models, the code allows employment of numerical wake potentials computed with electromagnetic (EM) field solvers. The corresponding impedances are fitted to a number of known analytical functions and the coefficients obtained in the fit are used as an input to the code. mbtrack performs a dynamic treatment of long-range resistive-wall and harmonic cavity fields, which are likely to be the two major factors impacting multibunch collective motions in many present and future ring-based light sources. Furthermore, it is capable of simulating beam-ion interactions as well as transverse bunch-by-bunch feedback. We describe the physical effects considered in the code and their implementation, which makes use of parallel processing to significantly shorten the computation time. mbtrack is benchmarked against other codes and applied to the MAX IV 3GeV ring as an example, where the importance of the interplay of various physical effects as well as coupling among different degrees of freedom is demonstrated.}
}

@article{Xu2019,
title = {Calculation of longitudinal collective instabilities with mbtrack-cuda},
journal = {Nuclear Instruments and Methods in Physics Research Section A: Accelerators, Spectrometers, Detectors and Associated Equipment},
volume = {922},
pages = {345-351},
year = {2019},
issn = {0168-9002},
doi = {https://doi.org/10.1016/j.nima.2019.01.041},
url = {https://www.sciencedirect.com/science/article/pii/S0168900219300774},
author = {Haisheng Xu and Uldis Locans and Andreas Adelmann and Lukas Stingelin},
keywords = {Collective instabilities, GPU computing},
abstract = {Macroparticle tracking is a prominent method for studying the collective beam instabilities in accelerators. However, the heavy computationalload often limits the capabilities of tracking codes. One widely used macroparticle tracking code for simulating collective instabilities in storage rings is mbtrack. The Message Passing Interface (MPI) has already been implemented in mbtrack to accelerate the simulations. However, many Central Processing Unit (CPU) threads are requested in mbtrack for the analyses of the coupled-bunch instabilities.Therefore, computer clusters or desktops with many CPU cores are needed. Since these are not always available, we employ a Graphics Processing Unit (GPU) with a CUDA programming interface as an alternative to run such simulations in a stand-alone workstation. All the heavy computations have been moved to the GPU. The benchmarks confirm that mbtrack-cuda can be used to analyze coupled-bunch instabilities of 484 bunches. Compared to mbtrack on an 8-core CPU, a 36-core CPU and a cluster, mbtrack-cuda is faster for simulations of up to 3 bunches. For 363 bunches, mbtrack-cuda requires approximately six times the execution time of the cluster and twice that of the 36-core CPU. The multibunch instability analysis demonstrates that the length of the ion-cleaning gap does not have a substantial influence, at least at 34 filling.}
}

@ARTICLE{Wang2023,
	author={Lei Wang and Jiancheng Yang and Mingxuan Chang and Fu Ma},
	title={GOAT: a simulation code for high intensity beams},
	keywords={Code development; Numerical methods; Beam dynamics; High-intensity effects},
	doi={https://doi.org/10.1007/s41365-023-01225-z},
	abstracts={A simulation code, GOAT, is developed to simulate single-bunch intensity-dependent effects and their interplay in the proton ring (pRing) of the Electron-Ion Collider in China (EicC) project. GOAT is a scalable and portable macroparticle tracking code written in Python and coded by object-oriented programming technology. It allows for transverse and longitudinal tracking, including impedance, space charge effect, electron cloud effect, and beam-beam interaction. In this paper, physical models and numerical approaches for the four types of high-intensity effects, together with the benchmark results obtained through other simulation codes or theories, are presented and discussed. In addition, a numerical application of the cross-talk simulation between the beam-beam interaction and transverse impedance is shown, and a dipole instability is observed below the respective instability threshold. Different mitigation measures implemented in the code are used to suppress the instability. The flexibility, completeness, and advancement demonstrate that GOAT is a powerful tool for beam dynamics studies in the EicC project or other high-intensity accelerators.},
	journal={Nuclear Science and Techniques},
     volume = {34},
     pages = {78},
    year = {2023},
    issn = {2210-3147},
   url ={https://doi.org/10.1007/s41365-023-01225-z}
}

@article{WANGDAN2022,
title = {Broadband impedance modeling and single bunch instabilities estimations of the advanced light source upgrade project},
journal = {Nuclear Instruments and Methods in Physics Research Section A: Accelerators, Spectrometers, Detectors and Associated Equipment},
volume = {1031},
pages = {166524},
year = {2022},
issn = {0168-9002},
doi = {https://doi.org/10.1016/j.nima.2022.166524},
url = {https://www.sciencedirect.com/science/article/pii/S016890022200136X},
author = {Dan Wang and Karl Bane and Derun Li and Tianhuan Luo and Olusola Omolayo and Gregory Penn and Stefano {De Santis} and Christoph Steier and Marco Venturini},
keywords = {Broadband impedance, Impedance modeling, Impedance budget, Pseudo-Green function, Single bunch instability, ALS-U project},
abstract = {The Advanced Light Source Upgrade (ALS-U) is a 4th generation diffraction-limited soft x-ray radiation source, consisting of a new accumulator ring (AR) and a new storage ring (SR). In both rings coupling-impedance driven instabilities need careful evaluation to ensure meeting the machine’s high-performance goals. This paper presents the workflow followed in building the impedance models and the beam-stability analysis based on those models. We follow the commonly accepted approach of separating the resistive-wall and the geometric parts of the impedance; the former is obtained by analytical formulas, the latter by numerical electro-magnetic codes (primarily CST Studio software) with perfectly-conducting boundary conditions. Impedance budgets are established and pseudo-Green functions calculated to be used in beam dynamics studies. We also present various ways to cross-check simulation results for reliable impedance modeling. Finally, the crucial single-bunch instability current thresholds for various operation modes are determined and discussed.}
}

@article{Carver2023,
  title = {Beam based characterization of the {European Synchrotron Radiation Facility Extremely Brilliant Source} short range wakefield model},
  author = {Carver, L. R. and Brochard, T. and Buratin, E. and Carmignani, N. and Ewald, F. and Hoummi, L. and Liuzzo, S. M. and Perron, T. and Roche, B. and White, S.},
  journal = {Phys. Rev. Accel. Beams},
  volume = {26},
  issue = {4},
  pages = {044402},
  numpages = {14},
  year = {2023},
  month = {Apr},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevAccelBeams.26.044402},
  url = {https://link.aps.org/doi/10.1103/PhysRevAccelBeams.26.044402}
}

@article{MALYSHEV2017,
title = {{RF} surface resistance study of non-evaporable getter coatings},
journal = {Nuclear Instruments and Methods in Physics Research Section A: Accelerators, Spectrometers, Detectors and Associated Equipment},
volume = {844},
pages = {99-107},
year = {2017},
issn = {0168-9002},
doi = {https://doi.org/10.1016/j.nima.2016.11.039},
url = {https://www.sciencedirect.com/science/article/pii/S0168900216311937},
author = {Oleg B. Malyshev and Lewis Gurran and Philippe Goudket and Kiril Marinov and Stuart Wilde and Reza Valizadeh and Graeme Burt},
keywords = {Surface resistance, Wakefield impedance, NEG coating, PVD},
abstract = {In many particle accelerators the beam parameters could be affected by the beam pipe wakefield impedance. It is vital to understand how the wakefield impedance might vary due to various coatings on the surface of the vacuum chamber, and this can be derived from surface resistance measurements. The bulk conductivity of two types of NEG films (dense and columnar) is determined. This is achieved by measuring the surface resistance of NEG-coated samples using an RF test cavity and fitting the experimental data to a standard theoretical model. The conductivity values obtained are then used to compare resistive wall wakefield effects in beam pipes coated with either of the two types of film.}
}

@misc{IW2D,
  author={Mounet, N.},
  title = {{ImpedanceWake2D}},
  howpublished = {\url{https://gitlab.cern.ch/IRIS/IW2D}}
}

@article{Yokoya1993,
    author = "Yokoya, Kaoru",
    title = "{Resistive wall impedance of beam pipes of general cross-section}",
    reportNumber = "KEK-PREPRINT-93-196",
    journal = "Part. Accel.",
    volume = "41",
    pages = "221--248",
    year = "1993"
}

@article{Migliorati2019,
  title = {Resistive wall impedance in elliptical multilayer vacuum chambers},
  author = {Migliorati, M. and Palumbo, L. and Zannini, C. and Biancacci, N. and Vaccaro, V. G.},
  journal = {Phys. Rev. Accel. Beams},
  volume = {22},
  issue = {12},
  pages = {121001},
  numpages = {16},
  year = {2019},
  month = {Dec},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevAccelBeams.22.121001},
  url = {https://link.aps.org/doi/10.1103/PhysRevAccelBeams.22.121001}
}

@book{Chao1993,
    author = "Chao, A.W.",
    title = "{Physics of collective beam instabilities in high-energy accelerators}",
    isbn = "978-0-471-55184-3",
    year = "1993"
}

@book{Ng2005,
author = {Ng, K Y},
title = {Physics of Intensity Dependent Beam Instabilities},
publisher = {WORLD SCIENTIFIC},
year = {2005},
doi = {10.1142/5835},
address = {},
edition   = {},
URL = {https://www.worldscientific.com/doi/abs/10.1142/5835},
eprint = {https://www.worldscientific.com/doi/pdf/10.1142/5835}
}

@article{SMALUK2018,
title = {Impedance computations and beam-based measurements: A problem of discrepancy},
journal = {Nuclear Instruments and Methods in Physics Research Section A: Accelerators, Spectrometers, Detectors and Associated Equipment},
volume = {888},
pages = {22-30},
year = {2018},
issn = {0168-9002},
doi = {https://doi.org/10.1016/j.nima.2018.01.047},
url = {https://www.sciencedirect.com/science/article/pii/S0168900218300640},
author = {Victor Smaluk},
keywords = {Cyclic accelerators and storage rings, Beams in particle accelerators, Beam dynamics, Collective effects and instabilities},
abstract = {High intensity of particle beams is crucial for high-performance operation of modern electron–positron storage rings, both colliders and light sources. The beam intensity is limited by the interaction of the beam with self-induced electromagnetic fields (wake fields) proportional to the vacuum chamber impedance. For a new accelerator project, the total broadband impedance is computed by element-wise wake-field simulations using computer codes. For a machine in operation, the impedance can be measured experimentally using beam-based techniques. In this article, a comparative analysis of impedance computations and beam-based measurements is presented for 15 electron–positron storage rings. The measured data and the predictions based on the computed impedance budgets show a significant discrepancy. Three possible reasons for the discrepancy are discussed: interference of the wake fields excited by a beam in adjacent components of the vacuum chamber, effect of computation mesh size, and effect of insufficient bandwidth of the computed impedance.}
}

@inproceedings{Bai2021,
  author       = {Z.H. Bai and G.Y. Feng and T.L. He and W. Li and W.W. Li and G. Liu and Z.L. Ren and L. Wang and P.H. Yang and S.C. Zhang and T. Zhang},
  title        = {{A Modified Hybrid 6BA Lattice for the HALF Storage Ring}},
  booktitle    = {Proc. IPAC'21},
  pages        = {407--409},
  eid          = {MOPAB112},
  keywords     = {lattice, emittance, damping, storage-ring, SRF},
  venue        = {Campinas, SP, Brazil},
  series       = {International Particle Accelerator Conference},
  number       = {12},
  publisher    = {JACoW Publishing, Geneva, Switzerland},
  month        = {08},
  year         = {2021},
  issn         = {2673-5490},
  isbn         = {978-3-95450-214-1},
  doi          = {10.18429/JACoW-IPAC2021-MOPAB112},
  url          = {https://jacow.org/ipac2021/papers/mopab112.pdf},
  note         = {https://doi.org/10.18429/JACoW-IPAC2021-MOPAB112},
  abstract     = {{In this paper, we propose a modified hybrid 6BA lattice as the baseline lattice of the Hefei Advanced Light Facility (HALF) storage ring. Similar to the Diamond-II lattice, the proposed lattice cell has one long straight section and one mid-straight section; but the two bend units adjacent to the mid-straight are LGB/RB units (LGB: longitudinal gradient bend, RB: reverse bend), which can give both lower emittance and shorter damping times. The designed HALF storage ring, with an energy of 2.2 GeV and 20 lattice cells, has a natural emittance of about 85 pm·rad.}},
}

@article{STABLE,
  title = {Graphics-processing-unit-accelerated simulation for longitudinal beam dynamics of arbitrary bunch trains in electron storage rings},
  author = {He, Tianlong and Bai, Zhenghe},
  journal = {Phys. Rev. Accel. Beams},
  volume = {24},
  issue = {10},
  pages = {104401},
  numpages = {13},
  year = {2021},
  month = {Oct},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevAccelBeams.24.104401},
  url = {https://link.aps.org/doi/10.1103/PhysRevAccelBeams.24.104401}
}

@misc{ELEGANT,
  title = {User’s manual for ELEGANT},
  howpublished = {\url{http://ops.aps.anl.gov/manuals/elegant_latest/elegant.html}}
}

@article{He2021,
  title = {Longitudinal equilibrium density distribution of arbitrary filled bunches in presence of a passive harmonic cavity and the short range wakefield},
  author = {He, Tianlong and Li, Weiwei and Bai, Zhenghe and Wang, Lin},
  journal = {Phys. Rev. Accel. Beams},
  volume = {24},
  issue = {4},
  pages = {044401},
  numpages = {12},
  year = {2021},
  month = {Apr},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevAccelBeams.24.044401},
  url = {https://link.aps.org/doi/10.1103/PhysRevAccelBeams.24.044401}
}

@article{He2022,
  title = {Periodic transient beam loading effect with passive harmonic cavities in electron storage rings},
  author = {He, Tianlong and Li, Weiwei and Bai, Zhenghe and Wang, Lin},
  journal = {Phys. Rev. Accel. Beams},
  volume = {25},
  issue = {2},
  pages = {024401},
  numpages = {13},
  year = {2022},
  month = {Feb},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevAccelBeams.25.024401},
  url = {https://link.aps.org/doi/10.1103/PhysRevAccelBeams.25.024401}
}

@InProceedings{Skripka2016b,
  author       = {G. Skripka and Å. Andersson and F.J. Cullinan and R. Nagaoka and P.F. Tavares},
  title        = {{I}mpedance {C}haracterization and {C}ollective {E}ffects in the {MAX} {IV} 3 {G}e{V} {R}ing},
  booktitle    = {Proc. of North American Particle Accelerator Conference (NAPAC'16),
                  Chicago, IL, USA, October 9-14, 2016},
  pages        = {843--846},
  paper        = {WEA3CO04},
  keywords     = {ion, impedance, synchrotron, feedback, experiment},
  venue        = {Chicago, IL, USA},
  series       = {North American Particle Accelerator Conference},
  number       = {3},
  publisher    = {JACoW},
  address      = {Geneva, Switzerland},
  month        = {Jan.},
  year         = {2017},
  isbn         = {978-3-95450-180-9},
  doi          = {https://doi.org/10.18429/JACoW-NAPAC2016-WEA3CO04},
  url          = {https://jacow.org/napac2016/papers/wea3co04.pdf},
  note         = {https://doi.org/10.18429/JACoW-NAPAC2016-WEA3CO04},
}

@inproceedings{brosi2023,
    author = {M. Brosi},
    title = {Time-resolved measurement and simulation of a longitudinal single-bunch instability at the {MAX IV 3 GeV ring}},
    booktitle = {Proc. IPAC'23},
    pages = {2642-2645},
    paper = {WEPA020},
    venue = {Venezia},
    series = {IPAC'23 - 14th International Particle Accelerator Conference},
    number = {14},
    publisher = {JACoW Publishing, Geneva, Switzerland},
    month = {05},
    year = {2023},
    issn = {2673-5490},
    isbn = {978-3-95450-231-8},
    doi = {doi:10.18429/jacow-ipac2023-wepa020},
    url = {https://indico.jacow.org/event/41/contributions/2223},
}


